Axiomatizing Resource Bounds for Measure

Resource-bounded measure is a generalization of classical Lebesgue measure that is useful in computational complexity. The central parameter of resource-bounded measure is the {\it resource bound} $\Delta$, which is a class of functions. When $\Delta$ is unrestricted, i.e., contains all functions with the specified domains and codomains, resource-bounded measure coincides with classical Lebesgue measure. On the other hand, when $\Delta$ contains functions satisfying some complexity constraint, resource-bounded measure imposes internal measure structure on a corresponding complexity class. Most applications of resource-bounded measure use only the "measure-zero/measure-one fragment" of the theory. For this fragment, $\Delta$ can be taken to be a class of type-one functions (e.g., from strings to rationals). However, in the full theory of resource-bounded measurability and measure, the resource bound $\Delta$ also contains type-two functionals. To date, both the full theory and its zero-one fragment have been developed in terms of a list of example resource bounds chosen for their apparent utility. This paper replaces this list-of-examples approach with a careful investigation of the conditions that suffice for a class $\Delta$ to be a resource bound. Our main theorem says that every class $\Delta$ that has the closure properties of Mehlhorn's basic feasible functionals is a resource bound for measure. We also prove that the type-2 versions of the time and space hierarchies that have been extensively used in resource-bounded measure have these closure properties. In the course of doing this, we prove theorems establishing that these time and space resource bounds are all robust.

==> numbering.tex <==
\usepackage{amsthm}

%% \newtheorem{theorem}{Theorem}[section]
%% \newtheorem{corollary}[theorem]{Corollary}
%% \newtheorem{lemma}[theorem]{Lemma}
%% \newtheorem{proposition}[theorem]{Proposition}
%% \newtheorem*{claim}{Claim}

\newenvironment{theorem_cite}[1]
{\begin{theorem}  {\rm (#1)}}
{\end{theorem}}
\newenvironment{lemma_cite}[1]
{\begin{lemma}  {\rm (#1)}}
{\end{lemma}}
\newenvironment{corollary_cite}[1]
{\begin{corollary}  {\rm (#1)}}
{\end{corollary}}
\newenvironment{proposition_cite}[1]
{\begin{proposition}  {\rm (#1)}}
{\end{proposition}}

\newenvironment{theorem_named}[1]
{\begin{theorem} {\rm (#1)}}
{\end{theorem}}
\newenvironment{lemma_named}[1]
{\begin{lemma} {\rm (#1)}}
{\end{lemma}}

\newenvironment{proof_claim}
{\noindent{\em Proof of Claim.}}
{\hfill $\square$ {\em Claim.}}

\newenvironment{Proof}
{\begin{proof}}
{\end{proof}}

\newenvironment{Proofnamed}[1]
{\begin{proof}[Proof #1.]}
{\end{proof}}

\newenvironment{pf}
{\begin{proof}[Pf.]}
{\end{proof}}

\newtheorem{observation}[theorem]{Observation}
\newtheorem{observations}[theorem]{Observations}

\newtheorem{openproblem}[theorem]{Open Problem}
\newtheorem{openquestion}[theorem]{Open Question}
\newtheorem{question}[theorem]{Question}

\newtheorem{fact}[theorem]{Fact}
\newtheorem{facts}[theorem]{Facts}

\newtheorem{problem}[theorem]{Problem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{definition}

\newtheorem*{definition}{Definition}
\newtheorem*{defn}{Definition}
\newtheorem*{definitions}{Definitions}

\newtheorem{example}[theorem]{Example}
\newtheorem{examples}[theorem]{Examples}
\newtheorem*{example*}{Example}
\newtheorem*{examples*}{Examples}

\newenvironment{example_cite}[1]
{\begin{example}  {\rm (#1)}}
{\end{example}}

\newtheorem{construction}[theorem]{Construction}
\newtheorem{extension}[theorem]{Extension}

\newtheorem*{remarks}{Remarks}
\newtheorem*{remark}{Remark}

\newtheorem*{notation}{Notation}
\newtheorem*{terminology}{Terminology}

\newtheorem*{ack}{Acknowledgment}
\newtheorem*{acks}{Acknowledgments}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\numberwithin{equation}{section}
\numberwithin{figure}{section}

